Market Integration of Excess Heat

Excess heat will be an important heat source in future carbon-neutral district heating systems. A barrier to excess heat integration is the lack of appropriate scheduling and pricing systems for these producers, which generally have small capacity and limited flexibility. In this work, we formulate and analyze two methods for scheduling and pricing excess heat producers: self-scheduling and market participation. In the former, a price signal is sent to excess heat producers, based on which they determine their optimal schedule. The latter approach allows excess heat producers to participate in a market clearing. In a realistic case study of the Copenhagen district heating system, we investigate market outcomes for the two excess heat integration paradigms under increasing excess heat penetration. An important conclusion is that in systems of high excess heat penetration, simple price signal methods will not suffice, and more sophisticated price signals or coordinated dispatch become a necessity.

==> Letter_list_of_changes.tex <==
% Summary of Revisions (mandatory)
% Upload a brief (one-page) document with a list of changes or a rebuttal against the points raised by the reviewers and the advocate when you submit the revised manuscript.

\section{Summary of revisions}
We addressed the typos pointed out by reviewer 2. We clarified some equations in the text, and defined some variables that we had not defined in the first submission. As correctly pointed out by reviewer 3, the github repository was empty. We updated the repository to contain our code, which can be used to reproduce our results. 

Reviewer 2 posed some broad questions : `Is there an estimate realistically of how much excess heat is as yet untapped in Copenhagen? How realistic in magnitude are the stylized case studies results?'. We addressed this feedback first of all in the introduction, where we added references to other works that estimate the excess heat potential in Copenhagen, as well as some other cities in Denmark. Furthermore, we put the case study excess heat penetration in perspective in Section III.B, by comparing the yearly scheduled excess heat to the estimated available excess heat as estimated by source [4] (Amer et al.). 

Reviewer 2 seemed to understand from our work that we consider unit commitment constraints. To clarify, we emphasize in Section II.A that our considered models are Linear Programs without any binaires. In Section II.B, we discuss that we do not consider unit commitment. In Section IV.B, we add suggestions for future work related to unit commitment and block bids.  

Reviewer 2 was also wondering whether Copenhagen currently allows excess heat producers to participate in the market. To address this comment, we summarize the current optimal dispatch and pricing mechanisms of district heating in Copenhagen in the introduction. 

Reviewer 2 comments that March 2020 was an abnormal month. We do not expect that load changes due to Covid in 2020 will affect our results qualitatively. Therefore, we decided not to address this comment. 

Finally, reviewer 2 commented that the usage of a Swedish price signal in a case study of Copenhagen may be . In response to this feedback, we added a comment in Section IV.B on sensitivity analysis on the scaling of Stockholm price signal.

The main feedback of reviewer 3 considered the modelling of heat network, including delays and losses. We add motivation for the lack of network constraints in our model in Section II.B. In the discussion section, we add a comment on how inclusion of delays and losses could affect our results, and indicate directions for future work. 
%Case study: place the added level of excess heat in perspective to estimates of excess heat potential in the area. 

Reviewer 3 asks how we deal uncertainty in market inputs. In this work, we do not consider the effect of uncertainty. We add this as a direction for future work. 

% Two comments we do not address:
% \begin{itemize}
%     \item `How would these results change if you did not pay excess heat producers in the self-scheduling case for heat that is wasted/not actually used in the market?' We don't find the question relevant: how could that work in practice? Also, figure 3 is ONLY the suboptimality due to suboptimal scheduling of the waste heat, it does not include what we PAY to the waste heat producers. Figure 6 is also only the market clearing price, it does not include the price paid to the ...
% \end{itemize}

==> sections/submitted_abstract.tex <==
\section{Context}
%\textbf{Waste heat is the future}
%District heating is expected to play an important role in future carbon neutral energy systems in urban areas. % \cite{Lund2014FourthGDH}. 
District heating networks facilitate the decarbonisation of heat generation, among others by allowing for distribution of waste heat to households. 
Examples of waste heat sources include supermarkets and data centers that produce heat as a by-product of cooling systems. %, as well as energy heavy industries such as cement factories. 
Compared to conventional sources, waste heat generators are generally smaller and less flexible. %of smaller capacity, and less flexible in their dispatch. %Waste heat generation is usually less flexible than conventional generation, as only limited deviation from a reference production profile is possible.
%It is expected that by XXXX, so much percent of heat will come from waste heat sources. 
Waste heat has only rarely been used, even though it is readily available in many areas and has been shown to decrease system cost and fuel usage when integrated \cite{Syri2015OpenDH}. A major barrier to its injection in district heating networks is the lack of suitable methods for pricing waste heat. %Research has focused on physical integration of waste heat sources into the system. 
It remains an open question how heat dispatch and pricing systems can be designed to optimally accommodate waste heat producers.

%\textbf{Stockholm price signal.}  
In the Open District Heating system of Stockholm, small waste heat producers are successfully integrated. %\footnote{\url{www.opendistrictheating.com}} 
They receive a price signal as a function of the ambient temperature, and then self-schedule their heat injection using a local optimization. This is a rather simple and computationally cheap way of scheduling waste heat. 
%The reasoning behind such pricing is that heat load is related to ambient temperature as well. 
%All heat injected by waste heat producers is accepted by the network operator. 
%\textbf{Participate in market clearing} 
Alternatively, smaller waste heat producers may participate in a heat market through an aggregator. The market would provide waste heat generators with an incentive to shift production to hours of high market prices, which would lower market prices. 

The question is under which circumstances it is beneficial to have the small waste heat producers participate in a market, both from the perspective of the system and of the market actors. 
To answer this question, we investigate the two ways of scheduling and pricing waste heat. %, and compare market outcomes based on different metrics. 

\section{Methodology}
We develop two methods for determining the dispatch schedule and price of waste heat generators. 

First, inspired by the Stockholm Open District Heating pricing system, we consider a case in which waste heat producers receive a heat price signal as a known function of the ambient temperature. In particular, the received price decreases with the ambient temperature, as heat load generally decreases with ambient temperature. Waste heat generators then determine an optimal generation schedule using a local self-scheduling problem. In this optimization problem, the waste heat generator's objective is to maximize profit, given electricity and heat price signals. 

Second, we formulate a district heating market clearing without network constraints as an linear optimization problem. The market-clearing results in scheduled quantities for all participants and a uniform market price. Bidding behavior of different market participants is modeled. For combined heat and power plants, we use the electricity price dependent bidding strategy as formulated in \cite{Mitridati2020Heat}. 
%In addition, we model the (bidding) behavior of waste heat producers under these two pricing systems. 
In particular, we consider supermarkets that produce heat as a by-product of their refrigeration system, which is driven by a heat pump. The supermarkets' flexibility in heat consumption and production is represented by modeling cooling cabinet heat dynamics as a set of linear equality and inequality constraints. Furthermore, we consider ambient temperature dependent coefficient of performance of the supermarkets.

\section{Case study and expected results}
%\textbf{what kind of case study}
We use the Copenhagen district heating system as a case study. 
The current system includes multiple combined heat and power plants, to which we add supermarket waste heat providers. We simulate a full year of hourly heat market outcomes, including dispatch schedules for conventional and waste heat producers, as well as market prices. Inputs used include total system heat load, electricity price from the Nord Pool, and ambient temperature.
For the self-scheduling problem, we use ambient temperature measurements and electricity prices. In both pricing methods, we consider the perfect forecast case for all inputs.

%\textbf{what kind of results expected}
We compare the outcomes of the two pricing methods to understand how the resulting schedules and revenues of the waste heat producers and conventional producers may differ. These differences are studied for different seasons. 
In particular, we are interested in ambient temperature dependencies of the dispatch schedules and heat prices. 
%Finally, we compare the total system costs of the two cases. 


==> setup/list_of_vars.tex <==
%%%%%%%%%%%%%% Sets
\nomenclature[S]{$\mathcal{T}$}{Set of time indices}
\nomenclature[S]{$\Gamma$}{Set of optimization variables}

%%%%%%%%%%%%% Indices
\nomenclature[I]{$i$}{Index for CHP generators}
\nomenclature[I]{$w$}{Index for \wh generators}
\nomenclature[I]{$t$}{Index for time periods}
\nomenclature[I]{$\mr{H}$}{Heat}
\nomenclature[I]{$\mr{E}$}{Electricity}

%%%%%%%%%%%%% Parameters
\nomenclature[P]{$\hat{L}$}{Forecasted heat demand [\si{\mega\watt\hour}]}
\nomenclature[P]{$c$}{Marginal production cost [\si{DKK/\mega\watt\hour}]}
\nomenclature[P]{$\cop_i$}{Coefficient of performance of heat pump [-]}
% CHP
\nomenclature[P]{$\alpha$}{Fuel price [DKK/\si{\liter}]}
\nomenclature[P]{$\mu$}{Fuel price [DKK/\si{\mega\watt\hour}]}
\nomenclature[P]{$\lambda\up{E}$}{Electricity spot price [DKK/ \si{\mega \watt \hour]}}
\nomenclature[P]{$r$}{Minimum power to heat ratio for CHP [-]}
% HP
\nomenclature[P]{$A$}{Cooled room parameter [-]}
\nomenclature[P]{$B$}{Cooled room parameter [\si{\celsius/\mega\watt}]}
\nomenclature[P]{$\Delta t$}{Time step [h]}
\nomenclature[P]{$T\up{A}$, $T\up{I}$}{Ambient/indoor temperature [\si{\celsius}]}
\nomenclature[P]{$R$}{Ramping limit [\si{\mega\watt\hour}]}
\nomenclature[P]{$\rho$}{Fuel efficiency [\si{\liter/\mega\watt\hour}]}
\nomenclature[P]{$F$}{Fuel intake [\si{\liter}]}


%%%%%%%%%%%%% Variables
\nomenclature[V]{$G$}{Generated energy [\si{\mega\watt\hour}]}
\nomenclature[V]{$L\up{E}$}{Heat pump electricity load [\si{\mega\watt\hour}]}
\nomenclature[V]{$W$}{Wasted energy [\si{\mega\watt\hour}]}
\nomenclature[V]{$P$}{Scheduled energy [\si{\mega\watt\hour}]}
% for heat network
\nomenclature[V]{$\lambda\up{H}$}{Heat market-clearing price [DKK / \si{\mega \watt \hour]}}
\nomenclature[V]{$C$}{Total production cost [\si{DKK}]}
\nomenclature[V]{$T\up{F}$}{Refrigerator temperature [\si{\celsius}]}

\printnomenclature





==> todo.tex <==
BIG TASKS
- make pictures explaining the 2 scheduling / pricing systems
- online appendix
- add to litrev

SMALL TASKS
- check that index has become e, not w

FINALLY
- send to Ida?



QUESTIONS TO JALAL
- could you check whether the short litrev I added is ok?
- added reference to line colors, you like?
- are labels ok now? 
- in fig 3, I made the y-axis same scale now. Do you like it? I am in doubt, because fig 3a now looks packed. 
- should I repeat the feasible regions I define in II-D in the appendices? (see red questions in appendix)
- any funding you would like to add? Feel free to do so in the Acknowledgement. Do you think it is ok the way I wrote it now?
- did I cite the data sources allright? (varmelast website in a footnote, 
